A Review of AI-enabled Routing Protocols for UAV Networks: Trends, Challenges, and Future Outlook

Unmanned Aerial Vehicles (UAVs), as a recently emerging technology, enabled a new breed of unprecedented applications in different domains. This technology's ongoing trend is departing from large remotely-controlled drones to networks of small autonomous drones to collectively complete intricate tasks time and cost-effectively. An important challenge is developing efficient sensing, communication, and control algorithms that can accommodate the requirements of highly dynamic UAV networks with heterogeneous mobility levels. Recently, the use of Artificial Intelligence (AI) in learning-based networking has gained momentum to harness the learning power of cognizant nodes to make more intelligent networking decisions by integrating computational intelligence into UAV networks. An important example of this trend is developing learning-powered routing protocols, where machine learning methods are used to model and predict topology evolution, channel status, traffic mobility, and environmental factors for enhanced routing. This paper reviews AI-enabled routing protocols designed primarily for aerial networks, including topology-predictive and self-adaptive learning-based routing algorithms, with an emphasis on accommodating highly-dynamic network topology. To this end, we justify the importance and adaptation of AI into UAV network communications. We also address, with an AI emphasis, the closely related topics of mobility and networking models for UAV networks, simulation tools and public datasets, and relations to UAV swarming, which serve to choose the right algorithm for each scenario. We conclude by presenting future trends, and the remaining challenges in AI-based UAV networking, for different aspects of routing, connectivity, topology control, security and privacy, energy efficiency, and spectrum sharing.

==> Excluded-text.tex <==
%Bring commented text here



%The following are a few recent survey papers published in 2020. One complete survey paper is \cite{survey1}, which focused on Software-Defined Network (SDN) and Network Function Virtualization (NFV) for UAV-assisted applications. It includes monitoring, cellular and satellite communications for drones. This paper also covered security aspects along with the relevant evaluation tools and future challenges of the UAV networks. In terms of routing, this survey focused on SDN-based routing. Although being very useful for SDN-based routing, this paper only focuses on Air-to-Ground methods.
%The most recent survey papers published in 2020 focused on routing aspects are the following. One complete survey paper recently issued is \cite{survey1}, which focus on Software-Defined Network (SDN) and Network Function Virtualization (NFV) for UAV-assisted applications.  It includes monitoring, cellular and satellite communications for drones. Also, it analyzes security aspects, as well as evaluation tools available and future challenges for UAV networks. In terms of routing, this survey focuses on SDN-based routing. Therefore, it does not covers many other types of UAV Networks, as for example A2A (Air-to-Air) communications.


%A survey of routing algorithms for flying ad hoc networks is provided in \cite{survey5}. This paper starts with UAV classification and communication applications, then follows with describing mobility models that are suitable for UAV networks. This paper classifies routing protocols based on how the routes are determined. The analysis of routing algorithms in this paper is thorough and deep. Nonetheless, it excludes an important class of routing algorithms, namely the learning-based routing algorithms, which offer superior performance for UAV-based applications. %Last, it includes challenges and open issues to research. A well-organized review of emerging routing protocols for UAV networks including the network architecture and design as well as the remaining issues is provided in \cite{survey6}. This paper offers a comparative study with advantages and disadvantages for each routing protocol to elucidate their applicability to UAV networks under different conditions. However, it includes only the position-based methods and does not consider many other algorithms such as proactive routing, reactive routing, and AI-enabled routing methods.

%In \cite{survey5}, the authors based the survey on routing in flying ad hoc networks. The paper starts with UAV classification and communication applications. It follows describing mobility models that are suitable for UAV applications. Then, it classifies routing protocols based on how routes are determined. This is a deep study in different routing protocols. However, we consider it misses learning-based routing algorithms, which are one of the best solutions for UAV-based applications. Last, it includes challenges and open issues to research. A well-described review of emerging routing protocols for UAV networks including network architecture and design and opening issues is introduced in \cite{survey6}. It offers a comparative study with advantages and disadvantages for each routing protocol, which helps analyzing its applicability in UAV networks. However, it includes only a position-based methods and does not consider many others like proactive, reactive, hybrid, AI-enabled methods.


%Another relevant survey paper is \cite{survey7}, which offers an exhaustive review of communication protocols, applications, and security issues of UAV-assisted networks. As appears from the paper title, the center of attention of this paper is UAV-assisted routing, which excludes a lot of routing approaches developed for a more general class of flying ad hoc networks. Similar to the last survey, \cite{survey4} is focused on routing protocols for UAV-aided vehicular ad hoc networks. Its main feature is the inclusion of advantages, disadvantages, application areas and future improvements for each routing protocol. Nevertheless, this paper only considers routing protocols for UAV-aided vehicular networks, not generic UAV networks. In summary, almost all of these previously published surveys do not pay enough attention to the emerging variants of AI-enabled routing protocols, which can be considered the most appropriate class of routing protocols for extremely dynamic UAV Networks.




%Another recent survey paper in UAV-assisted networks offers an exhaustive study in communications, applications and security \cite{survey7}. However, it focus centers its effort in UAV-assisted routing only, which misses a lot of opportunities in flying ad hoc networks. Similar to the last survey, \cite{survey4} focuses on routing protocols for UAV-aided vehicular ad hoc networks. Its main feature is the inclusion of advantages, disadvantages, application areas and future improvements for each routing protocol studied. Nevertheless, this paper only considers routing protocols for UAV-aided vehicular networks. In summary, all these previously published surveys lack of including AI-enabled routing protocols, which are the most appropriate methods for adapting to UAV Networks.







\begin{comment}
\begin{table*}[t]
\centering
\caption{Performance comparison table}
\label{performance_table}
{\footnotesize
\begin{tabular}{|P{2.2cm} | P{2.7cm} | P{0.75cm} | P{0.75cm} | P{1.4cm} | P{1.4cm} | P{7cm} |}
%\begin{tabular}{|l|l|l|l|l|}
\hline
\centering
\multirow{2}{*}{\textbf{Routing family}} & \multirow{2}{*}{\textbf{Algorithm}} &\multicolumn{4}{c|}{\textbf{Objective performance}} & \multirow{2}{*}{\textbf{Results}}\\\cline{3-6}
%\textbf{Routing family} & \textbf{Algorithm} &  \textbf{Objective performance} & \textbf{Results}\\
& & \textbf{Energy} & \textbf{Delay} & \textbf{Throughput} & \textbf{Connectivity} & \\
\hline
\multirow{7}{*}{Topology predictive} & PPMAC+RLSRP \cite{PPMAC} & & \checkmark & \checkmark & \checkmark & Compared to DMAC, LODMAC, OLSR, GPMOR, RARP, IMAC+OLSR:
\begin{itemize}
    \item Lowest network delay and longest path lifetime
    \item Highest route setup success and data delivery ratio.
    \item Better successful throughout without retransmissions.
\end{itemize} \\ \cline{2-7}
                                    & Predictive dijkstra's \cite{ArnauWiSEE, arnau2} & & \checkmark & & & Compared to conventional Dijkstra's algorithm: \begin{itemize}
                                        \item Up to 25\% decrease in end-to-end delay for 100 nodes.
                                        %\item Better enhancement for larger networks, higher node velocities and longer queueing times.
                                    \end{itemize} \\ \cline{2-7}
                                    & Predictive greedy routing \cite{greedySECON} & \checkmark & & \checkmark & & Compared to conventional Dijkstra's and static greedy:\begin{itemize}
                                        \item Higher probability of success (up to 100\%).
                                        \item Energy consumption reduction (up to 30\%). \end{itemize} \\ \cline{2-7}
                                    & P-OLSR \cite{rosati1, rosati2} & & & \checkmark & \checkmark & Compared to OLSR and BABEL: \begin{itemize}
                                        \item Cuts down the outage time by at least 85\%.
                                        \item Achieves a more stable goodput. \end{itemize} \\ \cline{2-7}
                                    & GPMOR \cite{GPMOR} & & \checkmark & \checkmark & & Compared to GPSR and GLSR: \begin{itemize}
                                        \item Better packet delivery ratio (up to 250\%).
                                        \item Lower average delay of the network (up to 50\%). \end{itemize} \\ \cline{2-7}
                                    & MPCA \cite{MPC} & & & \checkmark & \checkmark & Compared with LID, HD and WCA: \begin{itemize}
                                        \item Up to 500\% increase in clusterhead duration.
                                        \item Up to 70\% lower reaffiliation frequency. \end{itemize}\\ \cline{2-7}
                                    & RARP \cite{RARP} & & & \checkmark & \checkmark & Compared to conventional AODV: \begin{itemize}
                                        \item Up to 30\% increase in route setup success rate.
                                        \item Higher average path lifetime. \end{itemize}\\ \cline{2-7}
                                    & SFMPRGR \cite{imprvRGR2} & & \checkmark & \checkmark & & Compared to AODV, RGR, and MPRGR: \begin{itemize}
                                        \item 10\% increase in packet delivery ratio.
                                        \item 20\% reduction end-to-end delay. \end{itemize}\\ \cline{2-7}
                                    & PARRoT \cite{parrot} & & \checkmark & \checkmark & & Compared to AODV, OLSR, GPSR and B.A.T.M.A.N: \begin{itemize}
                                        \item Higher packet delivery ratio (at least by 45\%).
                                        \item Lower end-to-end latency \end{itemize}\\ 
\hline
\multirow{7}{*}{self-adaptive learning-based} & Adaptive Q-Routing Full-echo \cite{adap_q_routing} & & \checkmark & & & In comparison to Q-Routing and Dual Q-Routing: \begin{itemize}
    \item Smaller average delivery time.
\end{itemize}  \\ \cline{2-7}
                                    & AQRERM \cite{aqrerm} & & \checkmark & & & Compared to Q-Routing, DRQ-Routing and AQFE: \begin{itemize}
                                        \item Better overshoot and settling time of the learning.
                                        \item Lower average delivery time. \end{itemize} \\ \cline{2-7}
                                    & PBQ-Routing \cite{pbQ-Routing} & \checkmark & \checkmark & \checkmark & & Compared to Q‐Routing, Epi-R, PRoPHET and HBPR: \begin{itemize}
                                        \item Delivery probability almost gets doubled.
                                        \item Lower energy use and overhead reduced to half.\end{itemize} \\ \cline{2-7}
                                    & Q$^2$-Routing \cite{q2routing} & & \checkmark & \checkmark & & Compared to AODV and EQ-Routing: \begin{itemize}
                                        \item Lower packet delay.
                                        \item Higher packet success ratio.
                                        \end{itemize} \\ \cline{2-7}
                                    & DQ-Routing \cite{dQ-Routing} & & & \checkmark & & Compared to Q-Routing: \begin{itemize}
                                        \item Much higher average reward of DQ-routing.
                                        \item More likely to choose best action.
                                        \end{itemize}\\ \cline{2-7}
                                    & SAIFEQ-Routing & \checkmark & & \checkmark & & Compared to Q-R, REE-R, PE-R, AFEQ-R and SAHQ-R: \begin{itemize}
                                        \item Reduction in energy consumption between 7\% to 82\%.
                                        \item Increase of up to 264\% in packet delivery ratio.
                                        \end{itemize}\\ \cline{2-7}
                                    & ARdeep \cite{ardeep} & & \checkmark & \checkmark & & Compared to QGeo and conventional GPSR: \begin{itemize}
                                        \item Up to 30\% higher packet delivery ratio.
                                        \item Up to 30\% lower average end-to-end delay.
                                        \end{itemize}\\ \cline{2-7}
                                    & TQNGPSR \cite{TQNGPSR} & & \checkmark & \checkmark & & Compared with AODV, OLSR, GPSR, and QNGPSR: \begin{itemize}
                                        \item Outperforms in terms of the packet delivery ratio, end-to-end delay, and throughput.
                                        \end{itemize}\\ 
                                    
\hline
\end{tabular}
}
\end{table*}
\end{comment}


\begin{comment}
    \begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{figures/LCAD_routing.PNG}
	\caption{\footnotesize Load carry and deliver routing model \cite{routingreview2014}.}
    \label{LCDR_routing}
    \end{figure}
    
    \begin{figure}[h]
	\centering
	\includegraphics[width=1\columnwidth]{figures/cgsr_routing.PNG}
	\caption{\footnotesize CGSR routing model \cite{cgsr}.}
    \label{CGSR_routing}
    \end{figure}
\end{comment}


==> droneApps-longVersion.tex <==
\section{UAV technology: military, industrial and commercial drones} \label{sec:uavtech}
\arr{this section is under revision by Razi}

In this section, we review military, industrial and commercial drones with their applications and how the technology tends to grow in the next few years. 
Drones were originally utilized in risky missions and applications such as search and rescue, remote sensing in inaccessible areas, border control, homeland security, and military fields where UAVs could protect human life. However, noting the recent breakthroughs in drones' flight stability and reduced cost, long-range and feature-rich sensors and cameras, and addressing their safety, privacy, and security issues, drones have found their way into many commercial and personal applications, including shipping and delivery, inspections, aerial photography (e.g., 3D mapping) and entertainment, as illustrated in Figure \ref{uavtypes}. According to an economic report by the Association for Unmanned Vehicle Systems International (AUVSI), commercial drone technology is expected to reach the economic impact of tens of billion dollars by 2025 with the expected number of 100,000 jobs \cite{AUVSI}.


\begin{figure}[h]
 	\centering
	\includegraphics[width=1\columnwidth]{figures/uavtypes2.PNG}
	\caption{Military, industrial and commercial drones.}
    \label{uavtypes}
\end{figure}

\subsection{Military drones}

Drone technology initiated in the military domain, and often military-grade drones utilized more advanced technology, compared to industrial or commercial drones. Our focus on this paper is commercial drones, and we skip Drones used by the military range from small intelligence, surveillance and reconnaissance craft to medium-sized armed drones and large spy planes \cite{militarydrones1}. The idea of using drones in military environments is solving conflicts without involving humans into risky situation, as for example when executing high-profile missions. Due to the high convenience and the ability to reduce casualties so drastically, military sector invests high resources into research and development of military drones \cite{militarydrones2}.

UAVs in the military can be categorized based on their weight, range, speed and their specific capabilities. Based on their weight, we can differentiate class I, class II and class III drones. Class I refer to micro, mini or small drones that weight less than 150 kgs. Class II include tactical drones between 150 and 600 kgs. Last, class III are strategic drones weighting more than 600 kgs. Then, military drones are used in target and decoy, reconnaissance and combat applications, as well as for research and development.

Military drones are equipped with more complex technology, compared to industrial and commercial drones. For instance, we can find hyperspacial sensors, which use reflections to determine the material a target is made of by matching data collected by the sensors to unique fingerprints of each object. Also, multi-spectral targeting system with infrared sensors to combine multiple images forming one large image are used in long-range surveillance and high-altitude acquisition, tracking and range finding scenarios. Last, Light Detection and Ranging (LIDAR) sensing technology that measures distance by illuminating a target with a laser and analyzing the reflected light is commonly used in military drones \cite{militarydrones3}.



\subsection{Industrial drones}

Drones in industrial settings are used in a broad range of applications such as agriculture, mining, construction, energy and oil and gas. Industrial drones are typically equipped with different types of sensors including but not limited to LIDAR, GPS, range finders for collision avoidance, PIN diodes for motion detection and pressure gauges, which are all integrated with high definition cameras \cite{industrialdrone}. Also, environmental and climate sensors such as temperature, humidity, air pollution, and chemical sensors are embodied into industrial drones when necessary.
%Their function is to collect data in a sensor network with advanced image processing and uses artificial intelligence methods in regions that are not in range of human works. For example, areas where environmental conditions or dimensions make it hard for people to get access to them. For example, mines, factories and refineries which require maintenance periodically.

This approach realizes an aerial version of sensor networks to collect data from hard and inaccessible areas and use advanced image processing and AI methods for processing and decision making. Important examples include mines, factories, power plants, bridges, high-rise buildings and refineries which require maintenance periodically.

Considering the future trend of this technology, it is expected that industrial drones will extend their territory and will take over the majority of life-threatening tasks under complex circumstances \cite{industrialdrone1}. 



\subsection{Commercial drones}

Drones are used by ordinary people for regular tasks that range from hobby and entertainment to more complicated monitoring tasks. Commercial drones are useful and simplifying tools for collecting data remotely, especially in hard-to-reach areas and risky environment. The applications of commercial drones are countless and includes shipping and delivery, inspection, real state, security, insurance, life habitat monitoring, border patrolling, structural monitoring, entertainment, spots monitoring, fire monitoring, flood prediction, smart agriculture, forest monitoring, volcano monitoring, fishery, weather report, etc. 
Similar to industrial drones, commercial drones can also be equipped with different types of sensors such as LIDAR and high definition cameras. They can collect different types of information, such as visual data, thermal data, LIDAR data and multi-spectral data. Some deliverables from drone work include 3D maps, orthomosaics and actionable reports \cite{commercialdrone}. However, commercial drones must follow some regulations for their adequate use among other people. which are established by the Federal Aviation Administration (FAA).
For instance, in the US, commercial drones should have a maximum weight of 55 pounds and should operate at or below 400 feet above the ground when in uncontrolled (Class G) airspace, or obtain authorization before flying in controlled airspace (Class B, C, D, and E) \cite{faa}.


With technical capabilities evolving in the coming years, it is expected to observe more commercial drones being used in a wide range of applications to save money, improve safety, and increase efficiency of drone-based missions.

%can also be used in commercial applications with the purpose of collecting and delivering data. UAVs are a powerful tool for collecting data remotely without the need to expose humans to risky scenarios. Then, we find commercial drones in various applications, as shipping and delivering, inspection, real state, security and insurance. Commercial drones are composed of different types of sensors, but these are more limited to the ones used for data collection, such as LIDAR and high definition cameras. They can collect different types of information, such as visual data, thermal data, LIDAR data and multi-spectral data. Some deliverables from drone work include 3D maps, orthomosaics and actionable reports \cite{commercialdrone}. However, this type of commercial drones must follow some regulations for their adequate use among other people. which are established by the Federal Aviation Administration (FAA).

\subsection{Drone Manufacturers}
\textcolor{blue}{(Remove or take a more general approach to introduce the global market)}

A large portion of commercial drone market in the US, about 77\% of the market shares belongs to DJI company, but some other drone companies such as Intel, Vuneec, Parrot, GoPro, 3DR, HolyStone, Autel, SenseFly and Kespry complete the top 10 drone market shares in the US \cite{dronemanufacturers1}.

%Here is some vendors:
%1- 3D Robotics (3DR) Link: https://3drobotics.com/products/hardware/
%2- xFold http://www.xfoldrig.com/
%3- UAV America https://uavamerica.com/https://uavamerica.com/
%Skydio,GoPro,Teal,Altavian.,InstantEye Robotics.,Impossible Aerospace.VantageRobotics.


Also, many companies use drones to provide 3rd party aerial solution for different applications (e.g., Precision haws, a North Carolina-based company that offers smart agriculture solutions \cite{precisionhawk}). The number of these companies grows larger than 100 and a list of such companies can be found in \cite{uavcompanies}, where companies are classified into categories including hardware, drone delivery or drone racing companies, as an example.



==> future-old-long-ver.tex <==
\section{Future trends and remaining challenges}  \label{sec:futuredirections}
\fbox{This is the original longer version substantially revised by Razi.}

To satisfy UAV applications in critical and privacy-constrained scenarios, we must ensure the design of robust and secure communication protocols that exchange information between UAVs in a secure and energy-efficient way, among other requirements. However, current protocols need to invest time and money to safely satisfy all these needs.

\subsection{Trajectory datasets}

%UAVs face many challenges, not only due to their intrinsic and technological limitations, but also due to the design and networking constraints. Here, we study the drawbacks that prevent us from using UAVs successfully in different applications. We focus on communication and computation aspects, finding ways to solve these the critical challenges and issues.

In this section, we describe a list of areas that need further investigations. To complete this study, we provide future trends that can be applied to UAV networks as a solution to the remaining issues stated.
From communication perspective, UAVs face several challenges mainly arising from limited payload and a highly dynamic network topology. The following is a list of some challenges and issues \cite{challengescomm, challenges_comm, challenges_comp, challengessurvey, challengessurvey3}: 


\subsection{Connectivity}

UAV networks characterize by having high mobility nodes. Consequently, connectivity is one of the issues to solve. Establishing and maintaining connectivity between UAVs must be one of the objectives to perform accurate activities. Link failure in communication re-initiates the route discovery process that leads to packet delivery delay, data loss and network congestion with extra control packets. As the network lifetime is limited we must consider techniques that enhance link lifetime as long as possible. For example, connectivity-efficient methods must be considered when defining routing protocols by adding link remaining time or path lifetime into routing criteria \cite{survey4}.

Communication links between UAVs are extremely vulnerable due to the high varying network topology UAVs form. The links between UAVs can be created and lost frequently due to the changing positions of the UAVs, which results in intermittent links. Also, connectivity is dependent on interference caused by objects or environmental factors. Therefore, we must find a network topology and mobility model that considers this dynamicity with the goal to maintain connectivity the longest possible.

In some applications nodes are sparse in location, causing an intermittent connectivity. Also, UAVs can leave and join the network periodically because of malfunction or battery exhaustion. Therefore, connectivity must be considered a priority in the design work of the network, as well as applying the communication layers \cite{survey5}.




\subsection{Routing}

Routing for UAV Networks needs to adapt to high moving nodes with intermittent connectivity. In this survey, we studied AI-enabled routing protocols, which introduce techniques to incorporate or predict the nodes' mobility into the route selection process. However, routing protocols face many other challenges in order to be deployed in real efficient applications.

First, we note that most routing protocols consider a fully connected network whereas in reality link breakages exist, causing routing protocols to fail \cite{futurerouting1}.
Also, node mobility in routing protocols is tested in 2-dimensional spaces, whereas UAVs are expected to move in 3-dimensional spaces. Therefore, we must design a routing protocol that considers intermittent connectivity that is suitable for all three dimensions.

In security aspects, there are situations where some packets need to have more attention than others. For example, we can have some packets containing confidential information that need to be securely delivered to the destination in optimal timing. This is known as priority routing, where we deliver data based on priority. However, this raises another issue, as maintaining prioritized packet delivery options with other normal packet delivery at an optimal level is not treated in UAV routing protocols. Moreover, distributed networks add vulnerability to data exchange functions because it is easier to cyberattack a node rather than a central decision-maker. Cyberattacks targeting the network layer can be intended to capture and control packets in the network, introducing malicious nodes, and interrupting the routing operation. To address different network layer attacks in wireless networks, different secure routing schemes are introduced in \cite{futurerouting2}. Also, adding traditional cryptographic techniques to the data exchange process are not feasible for such resource-constrained and dynamic networks because it brings delay and computational resources in time and energy-constrained network scenarios. Therefore, the offered solutions do not adapt to UAV networks' dynamicity and resource constraints.
We need to incorporate protected messages that are secure in all network layers where priority routing is built on top of the routing algorithm.

In summary, we can state that designing a feasible and efficient routing protocol is challenging. Further work needs to be done towards a method that can offer promising results in sparse and highly dynamic flying ad hoc networks. 





\subsection{Energy}

The main energy source used by commercial UAVs is batteries, helping in mobility, control, transmission, data processing, and payload uses \cite{futureenergy1}. In current networking scenarios, the flight duration of UAVs is limited and insufficient to provide long-term continuous wireless network coverage \cite{futureenergy2, futureenergy3}, impacting on the communication performance of the network. As a result, operation mission, weather conditions and path conditions also affect energy consumption.  For this reason, we must optimize energy and power consumption in our communication protocol. UAV networks must incorporate power requirements as one of the crucial factors to be deployed in real applications. This means that power reduction techniques should be incorporated in the communication design of the network. In the design of UAV communication platforms, it is necessary to pay attention to effective energy collection mechanisms to prolong the network lifetime. For instance, in restricted areas where UAVs access to perform complicated tasks, we must make sure that energy is not a limitation to perform such activities. Therefore, extending network lifetime must be a design requirement in all scenarios. 

In UAV technology design to deal with the energy restriction bottleneck \cite{futureenergy4}, significant recent advances in battery technologies have been done, such as hydrogen fuel cells \cite{futureenergy5} and enhanced lithium-ion batteries \cite{6futureenergy}. Also, Radio Frequency (RF) transmission has enabled the new concept of Wireless Power Transfer (WPT) \cite{7futureenergy}, which provides controllable and sustainable energy supply for UAVs \cite{8futureenergy, 9futureenergy}. Nevertheless, further study needs to be done in order to improve the use of WPT by reducing the distance between charging stations and UAVs, the random energy arrivals, and the scalable nature of UAVs \cite{10futureenergy, 11futureenergy}. One research direction is considering mmWave communications for UAV networks, energy beamforming, and placement optimization of wireless charging stations. Integration into 5G, B5G and 6G are also research topics related to energy optimization.

In current routing protocols, only a small portion consider energy as a routing criterion. Therefore, when designing a routing protocol for UAV networks, we must consider the energy level in the decision-making criteria to extend the path lifetime accordingly. Further research needs to be done in energy-aware routing.
Last, one solution to reduce power consumption asks UAVs to store data and calculations for future analysis \cite{12futureenergy}, as well as group UAVs to reduce communication overlapping and duplicate data transmission.

\begin{table*}[t]
\centering
\caption{Remaining issues and future directions}
\label{remaining_issues}
{\footnotesize
\begin{tabular}{|p{2.3cm} | p{7cm} | p{8.5cm} |}
\hline
\centering
\textbf{Open issues} & \textbf{Problems} & \textbf{Future directions} \\
\hline
\begin{itemize}
\item Connectivity
\end{itemize} & \begin{itemize}
    \item Link failures bring limited network lifetime.
    \item Communication links between UAVs are extremely vulnerable.
\end{itemize} & \begin{itemize}
    \item Consider techniques that enhance link lifetime by adding link remaining time or path lifetime into routing criteria.
    \item Find a network topology and mobility model that considers this dynamicity with the goal to maintain connectivity the longest possible.
\end{itemize}\\
\hline
\begin{itemize}
\item Routing
\end{itemize} & \begin{itemize} 
\item Most routing protocols consider a fully connected network when in reality link breakages happen.
\item Prioritized and secure packet delivery option is not considered.
\item Cyberattacks can capture and control packets in the network.
\end{itemize} & \begin{itemize}
    \item Design a routing protocol that considers intermittent connectivity into the routing selection process, as well as 3-dimensional space.
    \item Incorporate protected messages that are secure in all network layers where priority routing is built on top of the routing algorithm.
\end{itemize}\\
\hline 
\begin{itemize}
\item Energy
\end{itemize} & \begin{itemize}
\item Flight duration of UAVs is limited, impacting on the communication performance of the network.
\item Battery designs are limited in energy optimization trends.
\item Only a small portion of routing protocols considers energy or power as a routing criteria. 
\end{itemize} & \begin{itemize}
\item Incorporate effective energy collection mechanisms to prolong the network lifetime as a design requirement.
\item Consider mmWave communications for UAV networks, energy beamforming and placement optimization of  wireless charging stations.
\item Examine energy-aware routing future directions to incorporate energy level in the decision-making criteria to extend path lifetime.
\end{itemize}\\
\hline
\begin{itemize}
\item AI integration
\end{itemize} & \begin{itemize}
\item Most networking solutions do not incorporate AI-based solutions.
\end{itemize} & \begin{itemize}
\item Applying ML, RL and DL techniques to routing, spectrum sharing, path planning, resource allocation and scheduling, as well as network prediction.
\end{itemize}\\
\hline
\begin{itemize}
\item Network security
\end{itemize} & \begin{itemize}
\item Jamming attacks occur by disrupting GPS signal causing loss of signal.
\end{itemize} &  \begin{itemize}
\item Incorporate machine learning methods to detect and eliminate jamming to provide a secure localization system.
\end{itemize}\\
\hline
\begin{itemize}
\item Radio spectrum
\end{itemize} & \begin{itemize}
\item Radio spectrum unavailability can cause the loss of command and control of the aircraft
\item Radio spectrum remains vulnerable to unintentional or intentional interference.
\end{itemize} & \begin{itemize}
\item Spectrum sharing and spectrum leasing techniques using advanced machine learning solutions.
\item Optimal communications including sensitivity to interference and adaptive antenna steering can optimize data acquisition objectives.
\end{itemize}\\
\hline
\begin{itemize}
\item Operational regulations
\end{itemize} & \begin{itemize}
\item Lack or ambiguity of regulations and standards for UAV operations.
\end{itemize} & \begin{itemize}
\item Develop certification standards and air traffic requirements for UAVs that include all regions in the worlds.
\end{itemize}\\
\hline
\end{tabular}
}
\end{table*}

\subsection{AI Integration}

Artificial intelligence (AI) integration in UAV networks is seen as one of the potential directions to efficiently use UAVs in many of the mentioned applications. AI is shown to be the best solution for autonomous UAVs within various kinds of networks \cite{futureAI1, futureAI2,futureAI3}. Moreover, it can also optimize network management and reduce their complexity \cite{futureAI4}. 
However, current networking designs are not fully deployed under artificial intelligence-based solutions. Therefore, future trends incorporate involving AI into UAV networks with the application of Machine Learning (ML) \cite{futureAI5}, Reinforcement Learning (RL) \cite{futureAI6}, and Deep Learning (DL) \cite{futureAI7}. As potential solutions, it is expected to help optimize routing, spectrum sharing, path planning, resource allocation and scheduling, enhancing network prediction, and overall boosting network performance for UAV networks. 




\subsection{Network security} 

Jamming attacks are considered common attacks to UAV networks \cite{jamming1}. Jamming refers to a deliberate interference signal generated by an adversarial node to block or disrupt a UAVs control or information channel. In UAV networks, where the localization system relies on GPS positioning, the GPS signal can be disrupted due to jamming, causing the UAV to lose the location, direction and speed tracking. Noting that GPS signals are not encrypted, it makes them vulnerable to jamming or other cyber-attacks to interfere with the UAVs positioning mechanism. To mitigate this problem, UAVs should contain other navigation or localization systems. For example, UAV localization methods are considered in \cite{uavlocalization}. Also, machine learning methods can be used to detect and eliminate jamming, or provide an additional reference for positioning verification \cite{jamming2}. 
    
\subsection{Radio spectrum} 

Enabling high-rate, low-latency and ultra-reliable wireless communications in UAV networks is a necessity to perform their large-scale usage in the future.
UAVs can be considered as a mobile platform for different computation and communication technologies. Currently, UAVs use different communication protocols and frequency bands to enable Air-to-Air (A2A) communications.
The main characteristic of the communication protocols used in UAV networks is that they offer a low-power wireless communication. Regardless of utilized technology, a proper management of spectrum access to minimize interference with ground networks is a key requirement of UAV networks. Radio spectrum unavailability or interference can cause the loss of command and control of the aircraft, which impacts the success of the mission. Also, the radio spectrum used by unmanned aircraft remains vulnerable to unintentional or intentional interference.
In recent years, progress has been made in obtaining additional dedicated radio-frequency spectrum (5030-5091 MHz) for drone operations \cite{cooney_2013}. Moreover, several methods are proposed to use spectrum sharing and spectrum leasing methods for UAV networks to improve the performance of data acquisition using UAV networks \cite{spectrum1, spectrum2}.
In a different line of research, some models using fiber optic communications \cite{fiberoptic}, laser \cite{laser} and LiFi \cite{lifi} have been proposed to provide a faster and more efficient way for transmitting large amounts of data over long distances to cover the increasing demand for bandwidth. These methods would relieve challenges for wireless networking with multiple UAVs such as bandwidth efficiency and security as they are more optimal a for high-density wireless data coverage in restricted areas.
However, more research is on the way to solve specific issues of optical communications including sensitivity to interference and adaptive antenna steering.
    
\subsection{Operational regulations} 

Another drawback in drone research and utilization is the lack or ambiguity of sufficient regulations and standards for UAV operations. This also includes the airspace designated for UAV operations, which is not currently regulated. The FAA must safely designate airspace for UAV flight operations, as well as develop certification standards and air traffic requirements for drones. Moreover, FAA must verify the safety of unmanned aircraft and related navigation procedures before integrating them into the national airspace. Consequently, test areas must be defined to ensure the appropriate functionality of UAVs in the airspace. Therefore, it needs to be a consensus between the affected organizations in order to have safer airspace for drones' missions. For example, international coordination is needed since different territories follow different standards and regulations. There are currently three different regions, which are region 1 that covers Europe, Africa and parts of the Middle East, region 2 that covers America and region 3 that covers Asia and the Pacific, which have different frequency bands for UAV operations. Also, these regulations should take into account different aspects such as flight safety, resident privacy and security. 


A summary of the remaining challenges and future trends that we reviewed here is included in Table \ref{remaining_issues}.


